Finite-Sum Smooth Optimization with SARAH

The total complexity (measured as the total number of gradient computations) of a stochastic first-order optimization algorithm that finds a first-order stationary point of a finite-sum smooth nonconvex objective function $F(w)=\frac{1}{n} \sum_{i=1}^n f_i(w)$ has been proven to be at least $\Omega(\sqrt{n}/\epsilon)$ for $n \leq \mathcal{O}(\epsilon^{-2})$ where $\epsilon$ denotes the attained accuracy $\mathbb{E}[ \|\nabla F(\tilde{w})\|^2] \leq \epsilon$ for the outputted approximation $\tilde{w}$ (Fang et al., 2018). In this paper, we provide a convergence analysis for a slightly modified version of the SARAH algorithm (Nguyen et al., 2017a;b) and achieve total complexity that matches the lower-bound worst case complexity in (Fang et al., 2018) up to a constant factor when $n \leq \mathcal{O}(\epsilon^{-2})$ for nonconvex problems. For convex optimization, we propose SARAH++ with sublinear convergence for general convex and linear convergence for strongly convex problems; and we provide a practical version for which numerical experiments on various datasets show an improved performance.

==> sections/experiments.tex <==
% \section{Discussions on SARAH++}\label{sec_discussion}

% \subsection{SARAH++ vs. SARAH+}\label{subsec_sarahpp_exp01}

% We proposed a new variant of SARAH called SARAH++ in the previous section. Note that SARAH++ only needs to tune $\eta$ while SARAH+ requires to tune both $\gamma$ and $\eta$. We also provided the theoretical convergence results for SARAH++ for the problem in \eqref{emperical_risk_loss} in the smooth convex cases. 

% We start this section by conducting experiments to show the advantages and performance of SARAH++ over SARAH+ on some popular datasets with diverse size $n$ such as \textit{covtype} ($n = 406,708$ training data) (estimate $L \simeq 1.90$), ijcnn1 ($n = 91,701$ training data) (estimate $L \simeq 1.77$), \textit{w8a} ($n = 49,749$ training data) (estimate $L \simeq 7.05$), and \textit{phishing} ($n = 7,738$ training data) (estimate $L \simeq 7.49$) from LIBSVM\footnote{http://www.csie.ntu.edu.tw/$\sim$cjlin/libsvmtools/datasets/} website. We consider $\ell_2$-regularized logistic regression problems with
% \begin{align*}
% f_i(w) = \log(1 + \exp(-y_i \langle x_i, w\rangle )) +
% \frac{\lambda}{2} \| w \|^2, \tagthis \label{eq_logistic_regression}
% \end{align*}
% where $\{x_i,y_i\}_{i=1}^n$ is the training data and the regularization parameter $\lambda$ is set to $1/n$, a widely-used
% value in  literature \cite{SAG,Nguyen2017_sarah}. We choose the parameters for SARAH+ with different values of $\gamma = \{1, \frac{1}{2}, \frac{1}{3}, \frac{1}{4}, \frac{1}{5}, \frac{1}{6}, \frac{1}{7}, \frac{1}{8}, \frac{1}{9}, \frac{1}{10}, \frac{1}{12} \}$ and $\{\frac{1}{2}, \frac{1}{3}, \frac{1}{4}, \frac{1}{5}, \frac{1}{6}, \frac{1}{7}, \frac{1}{8}, \frac{1}{9}, \frac{1}{10}, \frac{1}{12} \}$ and for SARAH++ with different values of $\eta = \{\frac{1}{2}, \frac{1}{3}, \frac{1}{4}, \frac{1}{5}, \frac{1}{6}, \frac{1}{7}, \frac{1}{8}, \frac{1}{9}, \frac{1}{10}, \frac{1}{12} \}$ and reported the best performance among them. For the maximum inner loop size $m$ for both algorithms, let us choose $m = 3n$. 
% % \begin{align*}
% %     \gamma & = \{1, \frac{1}{2}, \frac{1}{3}, \frac{1}{4}, \frac{1}{5}, \frac{1}{6}, \frac{1}{7}, \frac{1}{8}, \frac{1}{9}, \frac{1}{10}, \frac{1}{12} \} \\
% %     \eta &= \{ \frac{1}{L}, \frac{2}{3 L}, \frac{1}{2 L}, \frac{2}{5 L}, \frac{1}{3 L}, \frac{1}{4 L}, \frac{1}{5 L}, \frac{1}{6 L}, \frac{1}{8 L} \}
% % \end{align*}
% \begin{figure*}[!]
%  \centering
%  \includegraphics[width=0.33\textwidth]{Figs/covtype_I_01.png}
%  \includegraphics[width=0.33\textwidth]{Figs/ijcnn1_I_01.png}
%  \includegraphics[width=0.33\textwidth]{Figs/w8a_I_01.png} 
% %  \includegraphics[width=0.4\textwidth]{Figs/phishing_I_01.png} 
%   \caption{Comparisons of $\log[F(w) - F(w_*)]$ for SARAH+ and SARAH++ on \textit{covtype}, \textit{ijcnn1}, and \textit{w8a} datasets}
%   \label{fig_SARAHp_SARAHpp}
%  \end{figure*}
 
%  Figure~\ref{fig_SARAHp_SARAHpp} shows the comparisons between SARAH+ and SARAH++ for tuning hyper-parameters. Since SARAH+ has two parameters $\gamma$ and $\eta$ to tune, it is easy to see that, it could cover the parameter $\eta$ of SARAH++ by $\gamma = L\eta$. Hence, the performance of SARAH+ should not worst than SARAH++ if they tune properly both parameters $\gamma$ and $\eta$. In Figure~\ref{fig_SARAHp_SARAHpp}, we reported the value of $\log [ (F(w) - F(w_*)] $ for the $y$-axis and ``number of effective passes'' (or number of epochs) for the $x$-axis. The optimal solution of convex problem in \eqref{eq_logistic_regression} is found by using Gradient Descent with stopping criterion $\| \nabla F(w) \|^2 \leq 10^{-15}$. We observe that, the best performance of SARAH++ (with only tuning $\eta$) is comparable to the best performance of SARAH+ (with tuning both $\gamma$ and $\eta$) on \textit{covtype}, \textit{ijcnn1}, and \textit{w8a} datasets. 
 
% SARAH++ has a guarantee of the theoretical convergence (see Theorems~\ref{thm_general_convex_sarahpp} and \ref{thm_strongly_convex_sarahpp}) (while SARAH+ does not) and also requires to tune less parameters than SARAH+ with the similar performance. Therefore, it could be useful in both theory and practice. 
 
% \subsection{Stopping inner and outer iterations of SARAH++}\label{subsec_sarahpp_exp02}

% An interesting open question we would like to discuss here is the total complexity of SARAH++. Although we have shown the convergence results of SARAH++ in term of the iteration complexity in Section~\ref{sec_sarahpp}, the total complexity which is computed by the total number of evaluations of the component gradient functions still remains an open question. It is clear  that the total complexity would depend on the learning rate $\eta$ -- the factor that decides when to stop the inner iterations. 

% The total iterations $T$ can be understood as the total number of the updated iterations of the algorithm. \textbf{(May need to modify algorithm a bit -- should be easy - may put $G$ inside of inner loop)}. 

% The total complexity can be computed by $\sum_{i=1}^S (n + 2 (T_i - 1))$. If $T_i = 1$, $i = 1,\dots,S$, then it is obvious that the algorithm recovers GD algorithm with $T = \sum_{i=1}^S T_s = S$. Hence, the total complexities become $n S = \Ocal(\frac{n}{\epsilon})$ (in the general convex case) and $n S = \Ocal(n \kappa \log(\frac{1}{\epsilon}))$ (in the strongly convex case). 

% % Assume that every $T_i$ could achieve the same order of $T$, which are $\Ocal(\frac{1}{\epsilon})$ and $\Ocal(\kappa \log(\frac{1}{\epsilon}))$ for general convex and strongly convex, respectively. Then, the number of outer iterations $S$ could be $\Ocal(1)$ and hence the total complexity for SARAH++ in the best scenario could achieve $\mathcal{O}\left(n + \frac{1}{\epsilon} \right)$ and $\mathcal{O}\left(n + \kappa \log(\frac{1}{\epsilon}) \right)$ for general convex and strongly convex, respectively, as shown in Table~\ref{table_sarahpp}. This means that in the best scenario, it could achieve the best known total complexity results. Note that SVRG \cite{SVRG} and SARAH \cite{Nguyen2017_sarah} can achieve the total complexity of $\mathcal{O}\left((n + \kappa) \log(\frac{1}{\epsilon}) \right)$ in the strongly convex case for the finite-sum smooth optimization problems. 

% However, it is non-trival to derive the total complexity of SARAH++ since it depends on the learning rate $\eta$. We will leave this question as an open direction for the future research. 

% \begin{table} 
% \scriptsize
% \centering
% \caption{Summary of datasets used for experiments.}
% \label{table:datasets}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% Dataset  & $d$  & $n$ (train) & Sparsity  & $n$ (test)   & $L$ \\
% \hline \hline 
% \emph{covtype} & 54  & 406,709  & 22.12\% & 174,303 & 1.90396 \\
% \hline 
% \emph{ijcnn1} & 22  & 91, 701  & 59.09\% & 49, 990 & 1.77662 \\
% \hline
% \emph{news20} & 1,355,191  & 13, 997  & 0.03375\% & 5, 999 & 0.2500 \\
% \hline
% \emph{rcv1} & 47,236 & 677,399 & 0.1549\%  & 20,242 & 0.2500\\
% \hline 
% \end{tabular}
% %\captionsetup{justification=centering,margin=0.5cm}
% \end{table}

% Let us consider the following interesting results. \textbf{(will add later)}

% \begin{table}
%  \centering 
%  \scriptsize
% %\captionsetup{justification=centering,margin=0.0cm}
% \caption{Total complexity of SARAH++}
% \label{table_sarahpp}
% \begin{tabular}{|c|c|c| }
% \hline 
%  & \textbf{General Convex} & \textbf{Strongly Convex} \\
% \hline
% \hline
% Worst Scenario  & $\mathcal{O}\left(\frac{n}{\epsilon} \right)$ & $\Ocal(n \kappa \log(\frac{1}{\epsilon}))$ \\
% \hline
% Best Scenario  & $\mathcal{O}\left(n + \frac{1}{\epsilon} \right)$ & $\mathcal{O}\left(n + \kappa \log(\frac{1}{\epsilon}) \right)$ \\
% \hline
% \end{tabular}
% \end{table}

% \section{Numerical Experiments}\label{sec_experiments}

% \begin{itemize}
%     \item SARAH++ vs. SARAH+ on \textit{covtype}, \textit{ijcnn1}, \textit{w8a}, and \textit{phishing} datasets
%     \begin{itemize}
%         \item \textit{covtype}: 406,708 (data train), 174,304 (data test), 54 (features)
%         \item \textit{ijcnn1}: 91,701 (data train), 49,990 (data test), 22 (features)
%         \item \textit{w8a}: 49,749 (data train), 14,951 (data test), 300 (features)
%         \item \textit{phishing}: 7,738 (data train), 3,317 (data test), 68 (features)
%     \end{itemize}
%     \item Count stopping time of inner loop and outer loop for SARAH++ based on different $\eta$ and provide a conjecture (if possible)
% \end{itemize}





